REDriver: Runtime Enforcement for Autonomous Vehicles

Autonomous driving systems (ADSs) integrate sensing, perception, drive control, and several other critical tasks in autonomous vehicles, motivating research into techniques for assessing their safety. While there are several approaches for testing and analysing them in high-fidelity simulators, ADSs may still encounter additional critical scenarios beyond those covered once they are deployed on real roads. An additional level of confidence can be established by monitoring and enforcing critical properties when the ADS is running. Existing work, however, is only able to monitor simple safety properties (e.g., avoidance of collisions) and is limited to blunt enforcement mechanisms such as hitting the emergency brakes. In this work, we propose REDriver, a general and modular approach to runtime enforcement, in which users can specify a broad range of properties (e.g., national traffic laws) in a specification language based on signal temporal logic (STL). REDriver monitors the planned trajectory of the ADS based on a quantitative semantics of STL, and uses a gradient-driven algorithm to repair the trajectory when a violation of the specification is likely. We implemented REDriver for two versions of Apollo (i.e., a popular ADS), and subjected it to a benchmark of violations of Chinese traffic laws. The results show that REDriver significantly improves Apollo's conformance to the specification with minimal overhead.

==> proposition_back.tex <==
\begin{proposition}
\label{prop:alwaysincrease}
\textcolor{blue}{
    let $\varphi$ be a specification, $\pi$ be a trace, $x^k$ be the variable with the largest $\lvert D(\varphi, \pi, x^k) \rvert > 0$, $\pi'$ be the trace after the modification on $x^k$, and $\delta$ be a number larger than 0. Then,
    $$
    \forall \delta \geq \delta'> 0, x^k = D(\varphi, \pi, x^k) \cdot \delta' + x^k \implies \tilde{\rho}\left( \varphi, \pi' \right) > \tilde{\rho}\left( \varphi, \pi \right).
    $$
    % we can conclude $\rho(\varphi, \pi) \leq \rho(\varphi, \pi')$, where $\pi'$ is the trace after several repairs.
}
\end{proposition}


\begin{proof}
\textcolor{blue}{
Firstly, we explore the case when specification $\varphi$ is a Boolean Expression $\mu$. $\tilde \rho(\mu, \pi) = \rho(\mu, \pi)$ can be represented by a continuous function $f'(x_0,\cdots,x_n)$ as shown in Definition~\ref{def:Quantitative_Semantics}. Given that $f'(x_0,\cdots,x_n)$ is confined to linear or absolute value functions, the proposition holds for $\mu$.
}

\textcolor{blue}{
Then, we assume the proposition holds, and we can prove that the proposition holds if we can prove the proposition holds for each and every way $\varphi$ can be constructed, i.e., $\lnot \varphi_1$, $\varphi_1 \land \varphi_2$, $\varphi_1 \lor \varphi_2$, and $\varphi_1 \;\mathtt{U_I}\; \varphi_2$. 
}

\textcolor{blue}{
If $\varphi$ is in the format of $\lnot \varphi_1$, we have
$
\tilde\rho(\lnot \varphi_1, \pi) = - \tilde \rho(\varphi_1, \pi), 
$
 and
$
D(\lnot \varphi_1, \pi, x^k) = -D(\varphi_1, \pi, x^k).
$ 
Thus, by negating the modification, we can ensure that the proposition holds for $\lnot \varphi_1$.
}


\textcolor{blue}{
If $\varphi$ is in the format of $\varphi_1 \land \varphi_2$, 
$D(\varphi_1 \land \varphi_2, \pi, x^k) =
\frac{\partial \tilde \rho(\varphi_1 \land \varphi_2, \pi)}{\partial  \tilde \rho(\varphi_1, \pi)} \cdot D(\varphi_1, \pi, x^k) +  
\frac{\partial \tilde \rho(\varphi_1 \land \varphi_2, \pi)}{\partial  \tilde \rho(\varphi_2, \pi)} \cdot D(\varphi_2, \pi, x^k)
$. Suppose modifying $x^k$ by $\delta_1 \cdot D(\varphi_1, \pi, x^k)$ cause $\tilde \rho(\varphi_1, \pi)$ to increase, and modifying $x^k$ by $\delta_2 \cdot D(\varphi_2, \pi, x^k)$ cause $\tilde \rho(\varphi_2, \pi)$ to increase.
There are two situations. 
Firstly, if $\tilde \rho(\varphi_1, \pi) \neq \tilde \rho(\varphi_2, \pi)$, suppose $\tilde \rho(\varphi_1, \pi) > \tilde \rho(\varphi_2, \pi)$. Then, as shown in Definition~\ref{def:Gradient}, $\frac{\partial \tilde \rho(\varphi_1 \land \varphi_2, \pi)}{\partial  \tilde \rho(\varphi_2, \pi)} \gg \frac{\partial \tilde \rho(\varphi_1 \land \varphi_2, \pi)}{\partial  \tilde \rho(\varphi_1, \pi)}$. 
Hence, the modification to $x^k$ is $D(\varphi_1 \land \varphi_2, \pi, x^k) \cdot \delta \approx D(\varphi_2, \pi, x^k) \cdot \delta$. 
If $D(\varphi_1, \pi, x^k) \cdot D(\varphi_2, \pi, x^k) \geq 0$, the proposition obviously holds if $\delta \leq \delta_1$ and $\delta \leq \delta_2$. 
If $D(\varphi_1, \pi, x^k) \cdot D(\varphi_2, \pi, x^k) < 0$, ensuring $\delta < \frac{\tilde \rho(\varphi_1, \pi) - \tilde \rho(\varphi_2, \pi)}{-D(\varphi_1, \pi, x^k)}$, $\delta \leq \delta_1$ and $\delta \leq \delta_2$ guarantees the proposition holds.
Another situation is $\tilde \rho(\varphi_1, \pi) = \tilde \rho(\varphi_2, \pi)$. In this case, $D(\varphi_1 \land \varphi_2, \pi, x^k) =
\frac{D(\varphi_1, \pi, x^k)}{2} +  
\frac{D(\varphi_2, \pi, x^k)}{2}.
$ If $D(\varphi_1, \pi, x^k) \cdot D(\varphi_2, \pi, x^k) \geq 0$, the proposition obviously holds if $\delta \leq \delta_1$ and $\delta \leq \delta_2$. If $D(\varphi_1, \pi, x^k) \cdot D(\varphi_2, \pi, x^k) < 0$, the situation $D(\varphi_1, \pi, x^k) = - D(\varphi_2, \pi, x^k)$ indicates that the trace is impossible to fix since $D(\varphi, \pi, x^k) = 0$. 
Otherwise, 
% suppose $\lvert D(\varphi_1, \pi, x^k) \rvert > \lvert D(\varphi_2, \pi, x^k) \rvert$, the repair value is $\frac{D(\varphi_1, \pi, x^k) \cdot \delta}{2} + \frac{D(\varphi_2, \pi, x^k) \cdot \delta}{2}.$ 
by ensuring $\delta < \delta_1$ and $\delta < \delta_2$, we guarantee the proposition holds.
% The modification can increase the value of $\tilde \rho(\varphi_2, \pi)$.
}

\textcolor{blue}{
If $\varphi$ is in the format of $\varphi_1 \lor \varphi_2$, since $\varphi_1 \lor \varphi_2 =\lnot( \lnot \varphi_1 \land \lnot y)$,
we can deduce that the proposition always holds for $\varphi_1 \lor \varphi_2$.
}

\textcolor{blue}{
If $\varphi$ is in the format of $\varphi_1 \;\mathtt{U_I}\; \varphi_2$.
Since $\tilde \rho(\varphi_1 \;\mathtt{U_I}\; \varphi_2,\pi)$ is a combination of the function $\widetilde{max}$ and $\widetilde{min}$, we can deduce that the proposition always holds for $\varphi_1 \;\mathtt{U_I}\; \varphi_2$.
}

Therefore, we can conclude that the proposition holds.
\end{proof}
